A Perceptually-Validated Metric for Crowd Trajectory Quality Evaluation

Simulating crowds requires controlling a very large number of trajectories and is usually performed using crowd motion algorithms for which appropriate parameter values need to be found. The study of the relation between parametric values for simulation techniques and the quality of the resulting trajectories has been studied either through perceptual experiments or by comparison with real crowd trajectories. In this paper, we integrate both strategies. A quality metric, QF, is proposed to abstract from reference data while capturing the most salient features that affect the perception of trajectory realism. QF weights and combines cost functions that are based on several individual, local and global properties of trajectories. These trajectory features are selected from the literature and from interviews with experts. To validate the capacity of QF to capture perceived trajectory quality, we conduct an online experiment that demonstrates the high agreement between the automatic quality score and non-expert users. To further demonstrate the usefulness of QF, we use it in a data-free parameter tuning application able to tune any parametric microscopic crowd simulation model that outputs independent trajectories for characters. The learnt parameters for the tuned crowd motion model maintain the influence of the reference data which was used to weight the terms of QF.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> sec5-qualityfunction2.tex <==
% \ludo{Could be worth to define a number of terms that are used consistently used though the equations, e.g.$t$ represents the time of a single frame, $n$ is an individual character, $N$ is the total number of characters. This way you do not need to redefine them ni the table}
\begin{table}
    \centering
    \caption{Common terms for the equations in Table~\ref{tab:feature-eq}.}
    \begin{tabular}{cl}
         \toprule
         \textbf{Term} & \textbf{Definition} \\
         \midrule
         $s_i$ & Values of feature $i$ in the studied trajectory \\
         $r_i$ & Values of feature $i$ in reference data \\
         $T$ & Total number of time steps in the studied time window \\
         $t$ & Current time step \\
         $N$ & Total number of characters in the crowd \\
         $n$ & Index for the current characters \\
         $j$ & Index for each of the other characters \\
         \bottomrule
    \end{tabular}
    \label{tab:terms-eq}
\end{table}

\begin{sidewaystable*}
\centering
\caption{Measurements for the proposed trajectory features. Find in brackets where the definition for the terms is.}
\label{tab:feature-eq}
\begin{tabular}{llc}
\toprule
\textbf{Feature} & \textbf{Definition and terms} & \textbf{Equation}\\ 

\midrule
AWS &\makecell[l]{ Average walking speed of agent $n$, where $w_{n,t}$ is the current walking speed at time\\$t$ and $N$ is the number of characters in the crowd. } & $\mathcal{S}_{AWS} = \left\{ \sum_{t=0}^T{\frac{w_{n,t}}{T}} \right\}_n$\\

\midrule
\makecell[l]{DCS \\ DGD} &\makecell[l]{ Difference between walking speed, $w_{n,t}$, and comfort speed, $w_n^*$, of agent $n$ at time $t$. Same \\ equation for the difference between current direction, $\alpha_{n,t}$, and goal direction, $\alpha_n^*$. } & $\mathcal{S}_{DCS} = \left\{ w_n^* - w_{n,t} \right\}_{n,t}$ \\

\midrule
\makecell[l]{FSP \\ FDR} & \makecell[l]{ A time-invariant Gaussian filter $G$ is used to obtain $w_{n,t}^G$ and ${\alpha}_{n,t}^G$, and then subtracted to the \\ original high frequency speed and direction sequence, respectively.}  & $\mathcal{S}_{FSP} = \left\{ w_{n,t} - w_{n,t}^G \right\}_{n,t}$ \\

\midrule
AVL & \makecell[l]{ The smoothed sequence of direction of movements for each character $d_n^G$ is also used to \\ compute the total angular velocity feature value. } & $\mathcal{S}_{AVL} = \left\{ w_{t+1}^G - w_{t}^G \right\}_{n, t}$ \\

\midrule
LDN &\makecell[l]{ Number of characters $c_{n,t}$ inside an circle around each character $n$ at time $t$, divided by its area $a$. } & $\mathcal{S}_{LDN} = \left\{ \frac{c_{n,t}}{a} \right\}_{n,t}$ \\

\midrule
EDN &\makecell[l]{ Average pairwise distance, $d_{n,j}$, between character $n$ and all other characters at time $t$. } & $\mathcal{S}_{EDN} = \left\{ \sum_{j=1}^N{ \frac{d_{n,j}}{(N-1)}} \right\}_{n,t}$ \\

\midrule
\makecell[l]{DTA \\ DTO} & \makecell[l]{ Minimum distance between character $n$ and all other characters, $d_{n,j}$, or obstacles, $d_{n,o}$. } & $\mathcal{S}_{DTA} = \left\{ \min \left( \left\{ d_{n,j} \right\}_j \right) \right\}_{n,t}$ \\

\midrule
INE &\makecell[l]{ We compute the momentum of the linear system using the velocity, $w_{n,t}$, and mass, $m_{n}$. } & $\mathcal{S}_{INE} = \left\{ w_{n,t} * m_n \right\}_{n,t}$ \\

\midrule
IST &\makecell[l]{ Product between deviation because of neighbour $j$ and deviation from goal direction $d^*$. } & $\mathcal{S}_{IST} = a \left( \alpha_n, \alpha_{n,j} \right) * a(\alpha_n, \alpha_n^*)$ \\

\midrule
TCA &\makecell[l]{ Assuming linear motion, we compute relative velocity $v_{n,j}$ and position $p_{n,j}$ for each  \\  neighbour of character $n$. $\mathcal{S}_{TCA}$ is the minimum TTCA value for each character and frame. } & $\mathcal{S}_{TCA} = \left\{ min \left( - \frac{p_{n,j} * v_{n,j}}{ {\| v_{n,j} \|}^2} \right)_j \right\}_{n,t}$ \\

\midrule
\makecell[l]{DCA \\ TTC} &\makecell[l]{ Using TTCA, Distance at Closest Approach (DCA) is computed assuming linear movement. \\ Time to collision (TTC) is defined by the value of TTCA when DCA is under a threshold. } & $\mathcal{S}_{DCA} = \left\{ p_n + ttca_n * v_n \right\}_{n,t}$ \\

\midrule
IAN &\makecell[l]{ For future collisions (small DCA), product between TTCA and difference to desired direction $\alpha^*$. } & $\mathcal{S}_{IAN} = \left\{ {ttca}_n * (\alpha_n^* - \alpha_{n,t}) \right\}_{n,t}$ \\

\midrule
COL &\makecell[l]{ Number of times the distance $d_{n,j}$ between $n$ and $j$ is smaller than the sum of the radii, $r$. } & $\mathcal{S}_{COL} = \left\{ \sum_j{ \left[ d_{n,j} < r_n+r_j \right] }  \right\}_{n,t}$ \\

\midrule
OVP &\makecell[l]{ Total overlapping area between characters. Personal space radii depend on the application. } & $\mathcal{S}_{OVP} = \left\{ \sum_j{ ovp(n, j) }  \right\}_{n,t}$ \\

\midrule
LEN &\makecell[l]{ Length of the path, $l_n$, divided by the length of the line between the origin, $\hat{p}_0$, and goal, $\hat{p}_g$. } & $\mathcal{S}_{LEN} = \left\{ \frac{ l_n }{ \| \hat{p}_g - \hat{p}_0 \| } \right\}_{n}$ \\

\midrule
FDG &\makecell[l]{ Relation between density, $den_t$, and speed, $w_{n,t}$, in the trajectory and in real trajectories. $fd()$ \\ refers to the value of the fundamental diagram in real data.} & $\mathcal{S}_{FDG} = fd(den_t) - \frac{ \sum_t \sum_n{ w_{n,t} } }{ NTden_t }$ \\

\midrule
GLR &\makecell[l]{ Percentage of characters, $n$, that reach their goal, $\hat{p}_{n,g}$, in the studied time window [t, T]. } & $\mathcal{S}_{GLR} = \sum_n{ \left[ \hat{p}_{n,g} = \hat{p}_{n,T} \right] }$ \\
% \ludo{The equation suggests a sum more than a percentage, maybe check or rephrase}

\midrule
VAR &\makecell[l]{ Sum of differences between the variance for feature $i$ in reference, $\sigma_{i}$, and synthetic data, $\sigma_{s_i}$. } & $\mathcal{S}_{VAR} = \sum_i{ \| \sigma_{i} - \sigma_{s_i} \|  }$ \\
% \ludo{Should it be: between the variance $\sigma_{i}$ in real data and the feature value $s_i$ in synthetic data (i.e., for real data it's not a variance? but I might have misunderstood.}

\bottomrule
\end{tabular}
\end{sidewaystable*}

% \bea{Reference to definition containing definition of terms (enumeration). Say so in caption. Add table of definitions.}
